Unsupervised Segmentation in Real-World Images via Spelke Object Inference

Self-supervised, category-agnostic segmentation of real-world images is a challenging open problem in computer vision. Here, we show how to learn static grouping priors from motion self-supervision by building on the cognitive science concept of a Spelke Object: a set of physical stuff that moves together. We introduce the Excitatory-Inhibitory Segment Extraction Network (EISEN), which learns to extract pairwise affinity graphs for static scenes from motion-based training signals. EISEN then produces segments from affinities using a novel graph propagation and competition network. During training, objects that undergo correlated motion (such as robot arms and the objects they move) are decoupled by a bootstrapping process: EISEN explains away the motion of objects it has already learned to segment. We show that EISEN achieves a substantial improvement in the state of the art for self-supervised image segmentation on challenging synthetic and real-world robotics datasets.

==> Publicization/blog_and_tweets.tex <==
1. authors, title, website (w paper + code)

2. Twabstract: we take inspiration from dev psych of infant perception and neuro of recurrent perceptual grouping to dramatically improve SOTA in self-supervised segmentation. Main learning signal is object motion but works on static scenes.

3. Segmentation is fundamental to higher cognition, but our best models aren't very good

4. Why? Because they don't generalize to objects outside of their (supervised) training distributions.

5. That's weird. An object is first and foremost a physical thing, they shouldn't be invisible just because we haven't seen it before.

6. Also: we're losing to babies. Spelke/Carey/Baillergeon/etc.: young babies can infer object structure when things are moving, and by ~1 year they infer structure even when stuff isn't moving -- and they don't get supervision (at least not in the form of categorical pixel label maps.)

7. Overall this suggests we're missing something big: how do babies figure out what objects are in a category-agnostic way, without supervision?

8. The developmental trajectory gives a clue: motion not only reveals the structure of a scene (what's connected to what - Tsao & Tsao), but also hints at what sorts of things \textit{can} move independently of the rest of a scene -- ``Spelke objects.''

9. Thus a learning agent might learn what an ``object'' is -- and how to identify one in a static scene -- based on observing what moves.

10. Others (inculding us, PSGNet) have picked up on this idea of learning ``predicted common fate.'' But there's a problem with implementing it.
Most things that \textit{can} move are in fact \textit{not moving} at any given moment. Even a perfectly segmented map of the moving objects in a scene would have a lot of false negatives w.r.t. what \textit{can} move, which corrupts the learning signal.

11. The source of this problem is that grouping -- and Spelke objects -- are fundamentally \textit{relational} concepts. What is actually revealed when one sees a moving object? Instead of thinking about individual pixels/points/surface elemements, thing of \textit{pairs} of elements. 

12. If one element is moving and the other isn't, it can be inferred that they're on separate objects. And if two elements are moving around in lockstep, they're on the same object (common fate.) But what about pairs where \textit{neither} element is moving? In fact nothing is revealed about their connectivity. In trying to learn what an object is, an agent should just ignore those pairs.

13. We call this logic ``Spelke object inference.'' It's a way to learn what objects are without supervision, just motion. But because the learning signal is fundamentally relational, it really needs an architecture with a relational component to be learned.

14. Our second key innovation is to build such an architecture, which we call EISEN. The key training target of EISEN is a set of pairwise \textit{affinities} between each pair of spatial positions in the visual field. Intuitively, the affinity $(a,b)$ represents whether the scene elements $a$ and $b$ will move together -- i.e., belong to the same Spelke object.

15. Affinities encode the physical idea of a Spelke object, but they are not themselves a representation of objects. To extract actual object representations from affinities, we use a novel neural network that recurrently \textit{propagates and aligns} activation vectors over space via the affinities. It then \textit{selects groups of aligned vectors} -- which become the objects -- and \textit{suppresses redundant activity} with a winner-take-all mechanism.

16. Thus EISEN is an end-to-end differentiable neural network that extracts Spelke object segments from a single RGB image. It does this by estimating a physical connectivity graph (encoded as pairwise affinities) and then clustering this graph. It learns which pairs of things \textit{would} move together based on what is \textit{observed} moving together -- Spelke object motion is needed only for training, not for inference.

17. Combining these this architecture with Spelke object inference leads to a dramatic improvement in self-supervised object segmentation. EISEN is able to capture object details that other architectures miss on complex synthetic scenes; and on real-world scenes, such as the Bridge robotics dataset, it is able to segment the majority of Spelke objects in a scene where other architectures largely fail.

18. Training EISEN on Bridge exposes another challenge, which is that most realistic object motion in robotics-type settings is \textit{caused by an agent} -- in this case, the robot arm and gripper. This motion is \textit{correlated with an spatially adjacent to} that of the inanimate Spelke objects, so the two objects' motions need to be decoupled somehow.

19. We do this via a bootstrapping process: since EISEN sees the robot arm moving a lot more often than any other object, it naturally learns to segment it well first. Segments that have already been learned can be \textit{explained away} (i.e. subtracted) from the raw motion learning signal, leaving behind inanimate objects. In fact this is a general principle (not particular to robot arms or this dataset): objects that have been confidently segmented can top-down modify the raw training signal to improve it for further training.

20. [Future Directions] Other datasets, creating a full developmental program by not needing RAFT, using segments for other visual computations...

Notes

A. Having to implement Spelke object inference reveals what objects really are (Spelke objects at least): they're \textit{hypotheses about how the world could and will change.} That is, predicting that some set of pixels forms a (2D) object segment is really a guess that the physical elements covered by this segment will remain part of a coherent whole, at least in the near term. Cf. E.J. Green. While this idea doesn't directly apply to some things we call objects, like houses and street signs, it sort of makes sense at a higher conceptual level, in the sense that we expect all the parts of a house or a street sign to appear in concert, not separately (in most cases.)

As such, objects / segments are naturally part of one's \textit{world model}, which encodes one's theories of what is in the world (or a scene) and one's expectations of how stuff in the world behaves. See also Physical Scene Graphs.

B. The bootstrapping idea would also explain why we don't perceive inanimate held objects as part of the same entity as one's hands (given enough visual experience.) Though at a certain resolution, we might perceive a moving person and the objects they're holding as a single ``Spelke object.''


